Polygons of Finite Mutation Type

We classify Fano polygons with finite mutation class. This classification exploits a correspondence between Fano polygons and cluster algebras, refining the notion of singularity content due to Akhtar and Kasprzyk. We also introduce examples of cluster algebras associated to Fano polytopes in dimensions greater than two.

==> higher_dimensions.tex <==
% !TEX root = paper.tex
%----------------------------------------------------------------------
\section{Higher Dimensions}
\label{sec:higher_dimensions}
%----------------------------------------------------------------------

In this section we introduce examples extending the correspondence between cluster algebras and Fano polytopes to dimensions higher than two.

==> polygons.tex <==
% !TEX root = paper.tex

%----------------------------------------------------------------------
\section{Mutation of Fano polygons}
\label{sec:polygons}
%----------------------------------------------------------------------

In this section we demonstrate how to associate a cluster algebra to a Fano polygon $P$. We then show that the mutations (combinatorial and algebraic) are compatible with the definitions of mutation for seed-data (and quivers) and the birational maps $\mu_k$ respectively. To avoid overloading notation the Fano polygon $P$ lies in a lattice $\overline{M}$ for the rest of this section; this may be identified with the lattice $N$ in previous chapters.


\begin{dfn}
	\label{def:polygon_cluster_algebra}
	Given a Fano polygon $P$ by fixing the based lattice $N \cong \ZZ^m$ equipped with the skew-symmetric form from Definition~\ref{def:polygon_seed} let $E$ be the standard basis and $C$ be the standard generating set. We define the cluster algebra $\mathcal{C}_P$ associated to $P$ to be the cluster algebra generated by this seed. We define the \emph{unfrozen} cluster algebra associated to $P$ by forming the same seed $\bs = (\cE,C)$ and setting all frozen variables equal to $1$.
\end{dfn}

\noindent We refer to the quiver obtained from the exchange matrix of $\{\cdot,\cdot\}$ in this basis as $Q_P$. Unless we specify otherwise the `cluster algebra associated to $P$' shall refer to the \emph{unfrozen} cluster algebra. The importance of the `full' cluster algebra will not be explored in detail, but we do observe that we do not know of a counter-example to the following conjecture.


To prove that mutations of polygons induce the mutations of the corresponding seed, we need only show that the associated quivers are related by the appropriate mutation.



We now have a geometric reformulation of the notion of a \emph{maximally-mutable Laurent polynomial} in the surface case as an element of the \emph{upper cluster algebra} $\up(\mathcal{C})$ of $\mathcal{C}_P$. We recall CITE that the upper cluster algebra $\up(\mathcal{C})$ of a cluster algebra $\mathcal{C}$ is the intersection of the Laurent polynomial rings defined by its various clusters.

\begin{pro}
	Given a Laurent polynomial $f$ with support a Fano polygon $P$, $f$ is maximally mutable if and only if $\rho^\star f \in \up(\mathcal{C}_P)$, where we identify $\overline{N}$ with the image of $\rho$.
\end{pro}
\begin{proof}
	This is a tautology: by definition $f$ is maximally mutable if it remains Laurent under all possible mutations of $P$.
\end{proof}

\begin{rem}
	The upper cluster algebra may be identified with the global functions on the $\cA$ cluster variety of Fock--Goncharov~\cite{FG09}, that is, $\Gamma(\mathcal{A},\mathcal{O}_\mathcal{A})$. As we shall see in Section~\ref{sec:GHK_connection} there is also a very close connection to the `$\mathcal{X}$-cluster algebra', $\Gamma(\mathcal{X},\mathcal{O}_{\mathcal{X}})$.
\end{rem}

